Search for dark photon decays to $\mu^+\mu^-$ at NA62

The NA62 experiment at CERN, designed to study the ultra-rare decay $K^+ \to \pi^+\nu\overline{\nu}$, has also collected data in beam-dump mode. In this configuration, dark photons may be produced by protons dumped on an absorber and reach a decay volume beginning 80 m downstream. A search for dark photons decaying in flight to $\mu^+\mu^-$ pairs is reported, based on a sample of $1.4 \times 10^{17}$ protons on dump collected in 2021. No evidence for a dark photon signal is observed. A region of the parameter space is excluded at 90% CL, improving on previous experimental limits for dark photon masses between 215 and 550 MeV$/c^2$.

==> Tables/unusedtables/effiSignal_oldSel.tex <==
\begin{table}
    \caption{Summary of uncertainties and corrections to the signal selection efficiency.}
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        % variable 
        & \multicolumn{2}{c|}{$A^\prime\to\mu^+\mu^-$} \\ \hline
         Source & Uncertainty & Relative correction  \\
        \hline
        Statistics             & 2.1\% & --- \\
        NewCHOD association    & 0.6\% & $-1.2\%$ \\
        LKr association        & 0.5\% & $-4.5\%$ \\
        PID                    & \textcolor{red}{1.0\%} & \textcolor{red}{$-8.0\%$} \\
        Straw \textcolor{red}{quality and} resolution       & \textcolor{red}{1.5\%} &  --    \\ 
        Trigger                & 0.5\% & $-2.0\%$ \\
        LAV random veto        & 0.1\% & $-2.5\%$ \\
	   \hline 
	   Total                   & \textcolor{red}{2.9\%} & \textcolor{red}{$-17.1\%$} \\ \hline
    \end{tabular}
\label{tab:effi}
\end{table}

==> Tables/unusedtables/prompt_bkg_afterLAV.tex <==
\begin{table}
	\caption{Number of equivalent passing the 2 selections (including the LAV veto) for the 3 types of events discussed in text. The numbers in columns of Type-A and Type-C($\mu-K/\bar{p}$) are computed based on the ratio Type-B(after LAV)/Type-B(before LAV). }
	\centering
	\begin{tabular}{|c|c|c|c|c|c|}
	    \hline
		Selection & Type-A & Type-B & Type-C ($e-\mu$) & Type-C($\mu-K/\bar{p}$) & Total POT\\
		\hline
		Old & 0.065 & 0.02 & 0 & 0.005 & 0.072  \\
		New & 0.123 & 0.02 & 0 & 0.005 & 0.130  \\
		\hline
	\end{tabular}
	\label{tab:prompt_afterLAV}
\end{table}

==> Tables/unusedtables/prompt_bkg_beforeLAV.tex <==
\begin{table}
	\caption{Number of equivalent (raw) events passing the 2 selections (before the LAV veto) for the 3 types of events discussed in text. The last column gives the expected number of background events for the full statistics of the beam dump sample.}
	\centering
	\begin{tabular}{|c|c|c|c|c|}
	    \hline
		Selection & Type-A & Type-B & Type-C & Total POT\\
		\hline
		Old & 7.215(4) & 17.682(460) & 25.662(21) & 202.128 \\
		New & 7.138(4) & 9.253(345) & 4.307(3) & 131.328\\
		\hline
	\end{tabular}
	\label{tab:prompt_beforeLAV}
\end{table}

==> Tables/unusedtables/prompt_bkg_oldSel.tex <==
\begin{table}
	\centering	
	\caption{Expected number of events for $1.34\times 10^{17}$POT by type (columns 2-4) and overall (column 5). The LAV reduction related to column 3 is used in column 2 and on the 2 events $\mu-K/\bar{p}$ of column 4.}
	
	\begin{tabular}{|c|c|c|c|c|}
		\hline
		Selection & $\mu-\mu$ & $\mu-\pi$ & Other & Total\\
		% \hline
		% \textbf{Inactive Modes} & \textbf{Description}\\
		%\hhline{~--}
		\hline
		Before LAV & 115$\pm$ 67  & 35.36 $\pm$ 0.21  & 51 $\pm$ 12 & 202 $\pm$ 66 \\ \hline
		After LAV  &   0.065$\pm$  0.038  &  0.020 $\pm$ 0.002  &  0.002 $\pm$  0.001 &  0.087 $\pm$ 0.038\\ \hline
%		Before LAV & 115.440$\pm$ 66.560  & 35.366 $\pm$ 0.214  & 51.324 $\pm$ 11.773 & 202.128 $\pm$ 67.594 \\ \hline
%		After LAV  &   0.065$\pm$  0.038  &  0.020 $\pm$ 0.002  &  0.002 $\pm$  0.000 &  0.087 $\pm$ 0.038\\ \hline	
\end{tabular}
	\label{tab:prompt_oldSel}
\end{table}

==> Tables/unusedtables/tableAllRuns.tex <==
\begin{table}
    \caption{List of all good runs with the corresponding number of processed bursts and cumulative POT}
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
        % variable 
          Runs & N. of bursts & POT $\times 10^{16}$ & Average T10 $\times 10^{11}$ \\
        \hline
        11069 & 1174 & 0.78 & 67.1\\
        11070 & 420 &  0.29 & 70.7\\
        11071 & 1390 &  0.97 & 69.6\\
        11072 & 591 &  0.46 & 70.0\\
        11074 & 495 &  0.33 & 68.8\\
        11075 & 1415 &  0.98 & 69.6 \\
        11076 & 1115 &  0.77 & 69.3\\
        11077 & 187 & 0.13 & 69.8\\
        11078 & 1409 &  0.96 & 68.8\\
        11079 & 633 &  0.43 & 67.7\\
        11080 & 415 &  0.25 & 59.3 \\
        11082 & 398 &  0.26 & 65.0\\
        11083 & 1444 &  0.93 & 64.6 \\
        11084 & 1297 &  0.82 & 63.5\\
        11085 & 1416 &  0.92 & 65.0\\
        11086 & 1126 &  0.72 & 65.2\\
        11088 & 1343 &  0.85 & 63.3\\
        11089 & 1082 &  0.67 & 64.2\\
        11090 & 730 &  0.46 & 63.2\\
        11092 & 1369 &  0.85 & 62.2\\
        11093 & 1439 & 0.91  & 63.4\\
        11094 & 281 &  0.17 & 62.2\\
        \hline \hline
        22 runs & 21185 & 13.9 & 65.7\\
        
	   \hline 
    \end{tabular}
\label{tab:allruns}
\end{table}

==> Tables/unusedtables/tableCR_signalPollution.tex <==
\begin{table}
    \caption{Control region (CR) for the $\mu^+\mu^-$ search. Summary of expected di-muon events from combinatorial background ($N_\mathrm{exp}$), the related systematic error ($\delta N_\mathrm{exp}$), a number of possible observed events in data ($N_\mathrm{obs}$) and the $p$-value representing the probability to obtain a likelihood L for data-MC compatibility equal or worse than that corresponding to $N_\mathrm{obs}$ ($p(\mathrm{L}\leq \mathrm{L}_\mathrm{obs})$. In the last four rows a maximum signal pollution of 0.25 events is added to the expected background.}
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        % variable 
          $N_\mathrm{exp}\pm\delta N_\mathrm{exp}$ & $N_\mathrm{obs}$ & $p(\mathrm{L}\leq \mathrm{L}_\mathrm{obs})$ \\
        \hline

        $0.27\pm0.03$ & 0 & 1.0 \\
        $0.27\pm0.03$ & 1 & 0.23 \\
        $0.27\pm0.03$ & 2 & 0.030 \\
        $0.27\pm0.03$ & 3 & 0.0027 \\
 \hline
        $0.52\pm0.03$ & 0 & 1.0 \\
        $0.52\pm0.03$ & 1 & 0.40 \\
        $0.52\pm0.03$ & 2 & 0.096 \\
        $0.52\pm0.03$ & 3 & 0.015 \\
 \hline

	   \hline 
    \end{tabular}
\label{tab:CRPollution}
\end{table}

==> Tables/unusedtables/tableDiMuonCombinatorialAlternative.tex <==
\begin{table}
    \caption{\textcolor{red}{Summary of expected $\mu^+\mu^-$ events from combinatorial background ($N_\mathrm{exp}$), the related uncertainty ($\delta N_\mathrm{exp}$), the observed events in data ($N_\mathrm{obs}$) and 
    %the $P$-values representing the probability to count $N_\mathrm{obs}$ or more ($P_{N \geq N_\mathrm{obs}}$) and 
    the probability to obtain a likelihood L for data-MC compatibility equal or worse than that corresponding to $N_\mathrm{obs}$ ($P_{\mathrm{L}\leq \mathrm{L}_\mathrm{obs}}$). The data/MC ratio for same-sign events is used to determine the effective downscale factor.}}
    \centering
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        % variable 
          Region in CDA$_\mathrm{TAX}$ vs $Z_\mathrm{TAX}$ & $N_\mathrm{exp}\pm\delta N_\mathrm{exp}$ & $N_\mathrm{obs}$ 
          %& $p_{N \geq N_\mathrm{obs}}$ 
          & $p_{\mathrm{L}\leq \mathrm{L}_\mathrm{obs}}$ \\
        \hline
%             Outside CR & $44.1\pm5.0$ & 39 & 0.74 & 0.59 \\
%             CR$_3$ & $1.83\pm0.21$ & 2 & 0.55 & 0.71\\
%             CR$_2$ & $0.70\pm0.08$ & 1 & 0.50 & 0.50\\
%             CR$_1$ & $0.37\pm0.04$ & 1 & 0.31 & 0.31\\ 
%             CR$_{1+2+3}$ & $2.90\pm0.32$ & 4 & 0.33 & 0.55 \\ \hline
%             CR & $0.27\pm0.03$ & -- & -- & -- \\
%             SR & $0.027\pm0.003$ & -- & -- & -- \\ \hline

             Outside CR & $44.1\pm5.0$ & 39 &  0.59 \\
             CR$_3$ & $1.83\pm0.21$ & 2 &  0.71\\
             CR$_2$ & $0.70\pm0.08$ & 1 &  0.50\\
             CR$_1$ & $0.37\pm0.04$ & 1 &  0.31\\ 
             CR$_{1+2+3}$ & $2.90\pm0.32$ & 4 & 0.55 \\ \hline
             CR & $0.27\pm0.03$ & -- & -- \\
             SR & $0.027\pm0.003$ & -- & -- \\ \hline

	   \hline 
    \end{tabular}
\label{tab:DiMuonCombinatorialAlternative}
\end{table}

==> Tables/unusedtables/tableDiMuonCombinatorialBkg.tex <==
\begin{table}
    \caption{Summary of expected di-muon events from combinatorial background ($N_\mathrm{exp}$), the related systematic error ($\delta N_\mathrm{exp}$), the observed events in data ($N_\mathrm{obs}$) and the $p$-values representing the probability to count $N_\mathrm{obs}$ or more ($p(N \geq N_\mathrm{obs})$) and the probability to obtain a likelihood L for data-MC compatibility equal or worse than that corresponding to $N_\mathrm{obs}$ ($p(\mathrm{L}\leq \mathrm{L}_\mathrm{obs})$).}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        % variable 
          Mode & Region in CDA$_\mathrm{TAX}$ vs $Z_\mathrm{TAX}$ & $N_\mathrm{exp}\pm\delta N_\mathrm{exp}$ & $N_\mathrm{obs}$ & $p(N \geq N_\mathrm{obs})$ & $p(\mathrm{L}\leq \mathrm{L}_\mathrm{obs})$ \\
        \hline
                         & Outside CR & $61.4\pm9.2$ & 66 & 0.38 & 0.67\\
        $\mu^+\mu^+$     & CR & $0.40\pm0.06$ &  0 & 1.0 & 1.0 \\
                         & SR & $0.040\pm0.006$ & 0 & 1.0 & 1.0 \\ \hline
                         & Outside CR & $12.4\pm1.8$ & 13 & 0.47 & 0.80\\
        $\mu^-\mu^-$     & CR & $0.50\pm0.07$ & 0 & 1.0 & 1.0\\
                         & SR & $0.050\pm0.007$ & 0 & 1.0 & 1.0 \\ \hline
                         & Outside CR & $41.2\pm6.2$ & 39 & 0.61 & 0.87 \\
                         & CR$_3$ & $1.71\pm0.25$ & 2 & 0.51 & 0.69\\
        $\mu^+\mu^-$     & CR$_2$ & $0.65\pm0.10$ & 1 & 0.48 & 0.47\\
                         & CR$_1$ & $0.35\pm0.05$ & 1 & 0.29 & 0.30\\ 
                         & CR$_{1+2+3}$ & $2.71\pm0.27$ & 4 & 0.29 & 0.36 \\ \hline
        $\mu^+\mu^-$     & CR & $0.25\pm0.04$ & -- & -- & -- \\
                         & SR & $0.025\pm0.004$ & -- & -- & -- \\ \hline


	   \hline 
    \end{tabular}
\label{tab:DiMuonCombinatorial}
\end{table}

==> Tables/unusedtables/tableRefRuns.tex <==
\begin{table}
    \caption{Reference runs
    }
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        % variable 
          Runs & Reference run & L0TP granularity  \\
        \hline
        11069-11076 & 11071 & 6.25 ns \\
        11077-11080 & 11078 & 12.5 ns \\
        11082-11090 & 11083 & 25.0 ns \\
        11092-11094 & 11092 & 25.0 ns + New L0Calo T0 \\
	   \hline 
    \end{tabular}
\label{tab:refruns}
\end{table}

==> Tables/unusedtables/tableSignalMC.tex <==
\begin{table}
    \caption{Summary of grid-based, TAX-generated, dark-photon signal Monte Carlo productions.}
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
        % variable 
          Decay mode & Production mode & Number of mass points & Total number of events \\
        \hline
        $e^+e^-$     & Bremsstrahlung-like & 140 & $\simeq14$ M \\
        $e^+e^-$     & Meson-mediated      & 140 & $\simeq14$ M \\
        $\mu^+\mu^-$     & Bremsstrahlung-like & 98 & $\simeq13$ M \\
        $\mu^+\mu^-$     & Meson-mediated      & 98 & $\simeq13$ M \\ 

	   \hline 
    \end{tabular}
\label{tab:allMCs}
\end{table}
